Provable Limitations of Acquiring Meaning from Ungrounded Form: What Will Future Language Models Understand?

Language models trained on billions of tokens have recently led to unprecedented results on many NLP tasks. This success raises the question of whether, in principle, a system can ever ``understand'' raw text without access to some form of grounding. We formally investigate the abilities of ungrounded systems to acquire meaning. Our analysis focuses on the role of ``assertions'': textual contexts that provide indirect clues about the underlying semantics. We study whether assertions enable a system to emulate representations preserving semantic relations like equivalence. We find that assertions enable semantic emulation of languages that satisfy a strong notion of semantic transparency. However, for classes of languages where the same expression can take different values in different contexts, we show that emulation can become uncomputable. Finally, we discuss differences between our formal model and natural language, exploring how our results generalize to a modal setting and other semantic relations. Together, our results suggest that assertions in code or language do not provide sufficient signal to fully emulate semantic representations. We formalize ways in which ungrounded language models appear to be fundamentally limited in their ability to ``understand''.

==> v1/abstract.tex <==
Language models trained on billions of tokens have recently led to unprecedented results on many NLP tasks. This success raises the question of whether, in principle, a system can ever ``understand'' raw text without access to some form of grounding. 
We formally investigate the abilities of ungrounded systems to acquire meaning. Our analysis focuses on the role of ``assertions'': contexts within raw text that provide indirect clues about underlying semantics. We study whether assertions enable a system to emulate representations preserving semantic relations like equivalence. We find that assertions enable semantic emulation if all expressions in the language are referentially transparent. However, if the language uses non-transparent patterns like variable binding, we show that emulation can become an uncomputable problem. Finally, we discuss differences between our formal model and natural language, exploring how our results generalize to a modal setting and other semantic relations. Together, our results suggest that assertions in code or language do not provide sufficient signal to fully emulate semantic representations. We formalize ways in which ungrounded language models appear to be fundamentally limited in their ability to ``understand''.

==> v1/discussion.tex <==
\section{Stepping Back}
In this work, we formalized an argument that was raised by \citet{bk-2020} as a thought experiment.
\citet{bk-2020} question whether unsupervised training objectives are the right goal to chase for achieving natural language understanding. If meaning is defined as identifying which object in the real world, or which set of situations a linguistic element refers to, then, in a direct sense, an ungrounded system cannot understand meaning. But \citet{bk-2020} go further than this, claiming that an ungrounded system cannot even \emph{emulate} understanding because it is not clear how a system should learn to interpret strings, even if it can model their distribution. We formalize the notion of emulation as computing semantic relations that preserve semantic relations between underlying denotations.

% \will{Cite Wittgenstein language games in the paragraph above?}

One counterargument mentioned by \citet{bk-2020} is that indirect forms of grounding do exist in programming and natural language, which we formalize as assertions. The syntactic distributions of statements like \pythoninline{assert} allow us to indirectly observe semantic relations over the denotations. Assertions are one way that the distribution of strings in a corpus is not blind to their semantics.
% ---assertions provide one way to formalize this fact.
By studying them, we study whether this indirect grounding enables a computational system to emulate the underlying semantic relations.

% \paragraph{Are we ``Climbing the Right Hill''?}
\paragraph{Key Takeaways} While assertions do allow a system to emulate semantic relations in simple cases where the semantics are referentially transparent, we find that linguistic constructs like variable binding bring this task in conflict with the fundamental laws of computability. \upd{In other words, under our formal model of meaning and emulation, it is not just intractable for an ungrounded system to emulate understanding of a formal language, but, in some cases, \emph{impossible}.} We provide constructive examples where understanding must necessarily break down. We present these results in a formally precise framework building off formal approaches in logic, linguistics, and computer science. While we do not prove anything about natural languages, we do show that ungrounded models must fail to emulate equivalence in a very simple setting. \upd{A similar result likely extends to natural language understanding as well, which among other things, requires modeling referential identity (e.g., for sentences like \emph{Manny is the cat}).}
% the fact that our formal model is intuitively simpler than natural language suggests that our precise notion of impossibility (and perhaps a stronger one) also holds there.
Further, we believe much of our framework can be readily adopted in other works formalizing understanding in Turing-complete systems.

\paragraph{Open Questions}
% One future direction to further consider the emulation of relations besides equality---perhaps different relations would change the theoretical story in interesting ways.
% \roy{see comment above. changing equ to the word `equality' would make this sentence less confusing}. \nascomment{well, we kind of did, a bit.  maybe be a little more specific -- maybe there are particular properties of relations that would change the theoretical story in an interesting way?  }
What linguistic properties besides referential transparency relate to emulatability?
What is the role of uncertainty and ambiguity in this story? We view the extension in \autoref{sec:modal} as one step towards answering these questions, but there is more to be said.
In this work, we have focused on utterances, by default, as opposed to \emph{dialogues}. An exciting extension would be to formalize a dialogue between two speakers, interrupted by the ``octopus'' of \citet{bk-2020}.\footnote{\upd{The octopus thought experiment imagines a deep-sea octopus $O$ observes a dialogue between two humans by intercepting an underwater cable. Could $O$ learn to emulate the role of one of the speakers without exposure to life on land?}}
Existing theories of discourse could potentially be synthesized with this framework.
Finally, we have shown how emulating understanding fails from raw text alone within our setup. What is the minimal additional unit of meaning needed to resolve these issues?

% \roy{ This relates to the ``are we climbing the right hill'' question.}
% \roy{Another thing to think about: we have a total of 9 citations in this paper, 6 of them 2019-2020, 1 2011 and 2 very old. This would raise a serious concern for me as a reviewer that we haven't done our homework in terms of related work.}

==> v1/modal.tex <==
\section{Multiple Worlds} \label{sec:modal}

Programs execute in well-defined environments with a clear state. Speakers of natural language, on the other hand, have imperfect information and beliefs about the world around them. Thus, it can be more natural to model grounding context for language as a set of \emph{possible worlds}, rather than a single world state. We formalize this in two different ways (with two different physical interpretations) and explore how it affects our results.

Let $W$ be a set of all possible worlds.
We redefine denotations to be \textit{intensionalized} \citep{von2011intensional}, i.e., we write $\den{e}^w$ and $\den{e \mid \kappa}^w$ as denotations for some expression $e$ evaluated in world $w \in W$.
For a set of possible worlds $U \subseteq W$, we define contextual meaning as follows:

\begin{definition}[Modal contextualized meaning] \label{eq:modal-contextualized}
% TODO: Finalize this.
Let $U \subseteq W$. For all $e \in E(L)$, define $\den{\cdot}^U$ as
\begin{equation*}
    \den{e}^U = \{ \langle w, \den{e}^w \rangle \; \mid \; w \in U \} .
    % \mu^U(e) = \bigcup_{w \in U} \mu^w(e) .
\end{equation*}
\end{definition}

We need to define how the relation $=$ extends to meanings in this modal setting. We will do this in terms of a generic modal \emph{quantifier} $\odot : \{0, 1\}^{\abs{U}} \rightarrow \{0, 1\}$, which reduces a sequence of boolean values to a single boolean.

\begin{definition}[Modal semantic comparison] \label{eq:modal-comparison}
Let $U$ be a set of worlds, and $\odot$ a modal quantifier.
We compare two modal denotations as follows:
\begin{align*}
    \den{e}^U &=_\odot \den{e'}^U \iff \\
    \bigodot_{w \in U} \; \den{e}^U(w) &= \den{e'}^U(w).
\end{align*}
\end{definition}

% Note that this modified definition means $\mu^U$ is a relation ($\langle a, z, v \rangle \in \mu^U$) instead of a function of $a, z$ since the denotation can take different values in different worlds.
We will write the previously defined assertion oracle to apply in a specific world $w$, i.e. $\assert^w_=$. Similarly to $=_\odot$, we also extend it to quantify over multiple worlds:

\begin{definition}[Modal assertion oracle]
Let $U$ be a set of worlds, and $\odot$ a modal quantifier.
We overload $\assert^U_{=,\odot}$ for a set of worlds as follows:
\begin{equation*}
    \assert^U_{=,\odot}(e, e' \mid \kappa) = \bigodot_{w \in U} \assert^w_=(e, e' \mid \kappa) .
\end{equation*}
\end{definition}

We will consider two cases for $\odot$, either letting $\odot = \wedge$ (universal), or $\odot = \vee$ (existential). Each of these cases will have a different physical interpretation. With universal quantification, we will find that results analogous to \autoref{thm:transparency} and \autoref{thm:side-effects} hold. With existential quantification, it turns out that the equivalence class of $\mu$ is underspecified. In other words, not only is it impossible to compute an emulator, but there is not a single consistent way to emulate the underlying semantics.

\subsection{Universal Quantification}

In the first case we let $\odot = \wedge$. Two expressions are viewed as having the same meaning if they are equivalent in every possible belief world.
This is interpretable as observing text $L_\wedge$ written by a single author whose belief state is represented by multiple possible worlds. The author only asserts a statement is true if it is consistent across all worlds that they believe are possible.

In this case, it follows from \autoref{eq:modal-comparison} that the equivalence class of $\mu$ such that $\mu \cong_{=} \den{\cdot}^U$ is uniquely defined by $\assert^U_{=,\wedge}$.

\begin{theorem}
Fix $U \subseteq W$. Let $\odot = \wedge$. Consider $e, e' \in E(L)$. Then,
\begin{align*}
    \den{e}^U =_\wedge \den{e'}^U \iff \\
    \forall \kappa \in (\Sigma^*)^2, \; \assert_{=, \wedge} ^U(e, e' \mid \kappa) .
\end{align*}
\end{theorem}

\begin{proof}
Let $K = (\Sigma^*)^2$.
We start with the definition of modal semantic comparison:
\begin{align}
    \den{e}^U &=_\wedge \den{e'}^U \\
    &\iff \bigwedge_{w \in U} \den{e}^U(w) = \den{e'}^U(w) \\
    &\iff  \bigwedge_{w \in U} \bigwedge_{\kappa \in K} \den{e \mid \kappa}^w = \den{e' \mid \kappa}^w \\
    &\iff  \bigwedge_{w \in U} \bigwedge_{\kappa \in K} \assert_=^w(e, e' \mid \kappa) \\
    &\iff  \bigwedge_{\kappa \in K} \bigwedge_{w \in U} \assert_=^w(e, e' \mid \kappa) \label{eq:swap} \\
    &\iff  \bigwedge_{\kappa \in K} \assert_{=,\wedge}^U(e, e' \mid \kappa) \\
    &\iff  \forall \kappa \in K, \; \assert_{=, \wedge} ^U(e, e' \mid \kappa) .
\end{align}
\end{proof}

Crucial to this proof is the fact that we can swap the order of quantifiers in \eqref{eq:swap}. This holds only because $\odot = \wedge$.

\paragraph{Computability of $\mu$}
When each $\den{\cdot}^w$ is referentially transparent, an algorithm analogous to \autoref{fig:countable} can be used to compute a $\mu$ that emulates $\den{\cdot}^U$ with respect to $=_\wedge$. As the multiworld case generalizes the single world one, the same construction from \autoref{fig:countable} proves that $\mu$ can be uncomputable when side effects are allowed. Thus, results analogous to \autoref{thm:transparency} and \autoref{thm:side-effects} apply for $\assert^U_{=,\wedge}$.

\subsection{Existential Quantification}

In the second case we let $\odot = \vee$. Two expressions are viewed as having the same meaning if they are equivalent in \emph{some} world. This is interpretable as observing a large dataset of text $L_\vee$ generated by many authors, each with a different single belief world $w$. In the corpus, we imagine two expressions can be asserted to be equivalent in some context if \emph{any} of the authors would consider them to be equal in that context.

In this case, the equivalence class of $\den{\cdot}^U$ is not even well-defined by $\assert^U_{=,\vee}$. In other words, assertions do not disambiguate which notion of equivalence applies in the underlying semantics. This is a stronger sense in which meaning cannot be emulated from assertion queries. It is not just impossible to compute, but mathematically underspecified.

\begin{theorem}
Fix $U \subseteq W$. Let $\odot = \vee$.  Then, there exist a syntactic role $S$, expressions $e, e' \in E(S)$, and oracle function $\assert^U_{=, \vee}(e, e' \mid \kappa)$ such that both $\den{e}^U =_\vee \den{e'}^U$ and $\den{e}^U \neq_\vee \den{e'}^U$ are consistent with $\assert^U_{=, \vee}$.
\end{theorem}

\begin{proof}
Let $K = (\Sigma^*)^2$.
We construct a counterexample. Fix $U = \{w_1, w_2\}$, and fix two contexts $\kappa_1, \kappa_2$ in which both expressions can occur. We construct two versions of this modal setup, each specified by a table:

\begin{table}[t]
    \centering
    \begin{tabu}{|c|cc|c|[2pt]cc|c|}
        \hline
        & $w_1$ & $w_2$ & $\assert^U_{=,\vee}$ & $w_1$ & $w_2$ & $\assert^U_{=,\vee}$ \\
        \hline
        $\kappa_1$ & $0$ & $1$ & $1$ & $0$ & $1$ & $1$\\
        $\kappa_2$ & $1$ & $1$ & $1$ & $1$ & $0$ & $1$ \\
        \hline
        $\wedge_\kappa$ & $0$ & $1$ & $1$ & $0$ & $0$ & $0$ \\
        \hline
    \end{tabu}
    \caption{Two tables (separated by a thick line) representing two different versions of $U$. Within each table, each cell $\kappa, w$ in the main 2-by-2 grid contains the boolean value $\assert_=^w(e, e' \mid \kappa)$. The column to the right contains $\assert^U_{=,\vee}(e, e' \mid \kappa)$. Similarly, the row to the bottom records $\bigwedge_{\kappa \in K} \assert^w_{=,\vee}(e, e' \mid \kappa)$. Finally, the bottom right cell indicates whether $\den{e}^U =_\vee \den{e'}^U$.}
    \label{tab:ambiguity}
\end{table}

In both versions of the universe, the oracle function is the same. In particular, for the two possible contexts, we have:
\begin{align}
    \assert^U_{=, \vee}(e, e' \mid \kappa_1) &= 1 \\
    \assert^U_{=, \vee}(e, e' \mid \kappa_2) &= 1 .
\end{align}

\noindent However, in the left version, we have $\den{e}^U =_\vee \den{e'}^U$, whereas in the right one, $\den{e}^U \neq_\vee \den{e'}^U$. We can conclude that assertion queries do not uniquely determine the $=_\vee$ relation.
\end{proof}

As an equivalence class for $\mu$ is not even well-defined by $\assert^U_{=,\vee}$, we cannot hope to compute it from making queries. This is an even stronger sense in which it is impossible to preserve semantic equivalence using assertions.

In summary, if a corpus is internally consistent, representing a single world that all authors agree upon, and there are no side effects, we can expect to emulate representations preserving equivalence using assertions. Otherwise, there are various levels of formal challenges to accomplishing this emulation.

==> v1/other_relations.tex <==
\section{Other Semantic Relations} \label{sec:other-relations}

% https://plato.stanford.edu/entries/negation/#:~:text=Negation%20is%20in%20the%20first,and%20pragmatically%20in%20various%20ways.

Sections \ref{sec:no-side-effects}, \ref{sec:side-effects}, and \ref{sec:modal} investigate whether $\assert_=$ can be used to emulate meaning representations that preserve semantic equivalence. While equivalence is an important part of semantics, other semantic relations are also necessary for language understanding. In particular, the following feature prominently in theories of linguistic semantics:
\begin{itemize}
    \item \textbf{Entailment} In general terms, an entailment \citep{winter_2016} relation $\rightarrow$ is a partial order over $Y$. Intuitively, if $y \rightarrow y'$, then $y$ is a ``special case'' of $y'$. For example, one could construct a semantic analysis of English where the following holds:
    \begin{equation}
        \den{\textrm{fat cat} \mid \textrm{a}, \textrm{sits}} \rightarrow \den{\textrm{cat} \mid \textrm{a}, \textrm{sits}} .
    \end{equation}
    \item \textbf{Contrary negation} Negation is a complex topic in semantics. One sense of negation is if two meaning representations are ``contrary'' \citep{sep-negation}, meaning both cannot be true at the same time, although one being true does not necessarily imply the other is false. Formally, let each $y \in Y$ be a set. We say that $y \contrary y'$ ($y$ is contrary to $y'$) iff $y \cap y' = \emptyset$. Algebraically, $\contrary$ is symmetric and anti-reflexive.
\end{itemize}

Recall from \autoref{def:equal-hat} that we extend a generic relation $\rel$ from $\den{\cdot \mid \kappa}$ to $\den{\cdot}$ by defining $\den{e} \rel \den{e'}$ iff, for all $\kappa \in (\Sigma^*)^2$,
\begin{align}
    \den{e \mid \kappa} &= \den{e' \mid \kappa} = \emptyset \\
    \vee \quad \den{e \mid \kappa} &\rel \den{e' \mid \kappa} .
\end{align}

Can assertions about such relations be used to compute some $\mu$ emulating $\den{\cdot}$ with respect to $\rel$? For a referentially transparent language, the answer is yes.

\begin{theorem} \label{thm:all-rel}
Consider $L$ such that each $e \in E(L)$ is referentially transparent.
Consider a semantic relation $\rel : Y^2$.
Then, there
exists $\mu : E(L) \rightarrow M$
such that $\mu$ emulates $\den{\cdot}$ w.r.t. $\rel$.
% Then, there exists $\mu : \Sigma^* \rightarrow M$ and some Turing machine $T$ with oracle access to $\assert_\rel^*$ such that,
% for each support $D \subseteq (\Sigma^*)^2$,
% $\mu$ emulates $\den{\cdot}$ w.r.t. $\rel$ over $\suppset{D}_L$,
% $\mu \cong_\rel \den{\cdot}$,
% $\rel$ is decidable over $M$,
% and, for all $e \in E(L)$, $T$ computes $\mu(e)$ on input $e$.
% and $\mu(e) \stackrel{?}{\rel} \mu(e')$ is decidable.
\end{theorem}

\begin{proof}
% Assume without loss of generality that $L$ is a language defined over the alphabet $\{0, 1\}$.
Similarly to \autoref{thm:transparency}, we present the proof constructively as a Python program to compute $\mu : E(L) \rightarrow M$, where $M$ is an arbitrary space of representations. We then show how $\rel$ is defined over $M$, completing the proof that $\mu \cong_{\rel} \den{\cdot}$ over $E(S)$ for any syntactic role $S$.

\autoref{fig:extended-countable} shows the algorithm to compute $\mu(e) \in M$. In Python, $\mu(e)$ is a dictionary; we interpret it as a function $\mu(e) : \Sigma^* \times \Sigma^* \rightarrow \{0, 1, \emptyset\}$, where $\emptyset$ represents values that are not set. Define $\rel$ over $\mu(e) \in M$ as follows:
\begin{align}
    \mu(e) &\rel \mu(e') \iff \\
    &\begin{cases}
        \label{eq:cases}
        \mu(e)(e, e') & \textrm{if} \; \mu(e)(e, e') \neq \emptyset \\
        \mu(e')(e, e') & \textrm{if} \; \mu(e')(e, e') \neq \emptyset .
    \end{cases}
\end{align}

The only way for both $\mu(e)(e, e') \neq \emptyset$ and $\mu(e')(e, e') \neq \emptyset$ is if $e = e'$. Otherwise, one of these values will be null.
% \nascomment{I had a hard time making the above line intuitive.  I think there's a case where the meaning is not clear; suppose $\mu(e')(e, e')$ and $\mu(e)(e,e')$ are both not null, but $\mu(e)(e,e') \not = \mu(e')(e, e')$?}

% The loop variable \pythoninline{cand} in \autoref{fig:extended-countable}
In \autoref{fig:extended-countable}, \pythoninline{cand}
either reaches $e$ before $e'$, or $e'$ before $e$. By symmetry of \eqref{eq:cases}, assume it reaches $e$ before $e'$. Then $\mu(e')(e, e') \neq \emptyset$, so 
\begin{align}
    \mu(e) \rel \mu(e') &\iff \mu(e')(e, e') = 1 \\
    &\iff \assert_\rel(e, e' \mid \lambda^2) = 1 \\
    &\iff \den{e} \rel \den{e'} .
\end{align}
\noindent Therefore $\mu \cong_\rel \den{\cdot}$ over $E(S)$.
\end{proof}

\begin{figure*}
    \centering
    \begin{python}
from typing import Callable, Dict, Tuple
    
AssertType = Callable[[str, str, str, str], bool]

def emulate(expr: str, ass_rel: AssertType) -> Dict[Tuple[str, str], bool]:
    repres = {}
    for cand in all_strings():
        repres[expr, cand] = ass_rel(expr, cand, "", "")
        repres[cand, expr] = ass_rel(cand, expr, "", "")
        if expr == cand:
            return repres
    \end{python}
    \caption{\pythoninline{emulate} computes a structured representation of the input string \pythoninline{expr} that preserves any semantic relation $\rel$ in terms of assertion queries. The iterable \pythoninline{all\_strings} is defined in \autoref{fig:subroutines}.}
    \label{fig:extended-countable}
\end{figure*}

The reason why we need to modify \autoref{thm:all-rel} compared to \autoref{thm:transparency} is that, here, $\rel$ is not an equivalence relation. In \autoref{thm:transparency}, going from \eqref{eq:pre-equiv-rel} to \eqref{eq:equiv-rel} relied on reflexivity, transitivity, and symmetry: the three properties that constitute equivalence. This modification significantly enlarges the size of the representations in $M$. Rather than representing each $e$ with an integer $i \in \mathbb{N}$, $\mu(e)$ becomes a dictionary comparing $e$ to all strings reached before it in the enumeration. This represents an increase in space complexity from linear to exponential in the length of $e$.

==> v1/preliminaries.tex <==
\section{Preliminaries}

Let $L \subseteq \Sigma^*$ denote a formal language over alphabet $\Sigma$.
% We refer to $e \in \Sigma^*$ as a \textit{substring} of $L$ if there exist $a,z \in \Sigma^*$ such that $aez \in L$. By $E(L)$, we denote the set of substrings of $L$.
% We will generally use $x$ to denote any full string in $L$, and $e$ any string in $\Sigma^*$. 
We will use $\lambda$ to denote the empty string.

Let $(\Sigma^*)^2$ denote the Cartesian product of $\Sigma^*$ with itself; i.e., the set of all pairs of strings.
Resembling \citet{clark2010three}, we refer to a tuple $\langle l, r \rangle \in (\Sigma^*)^2$ as a syntactic \emph{context}. We also use other symbols to refer to a context, e.g., $\kappa = \langle l, r \rangle$. We denote by $\lambda^2$ the empty context $\langle \lambda, \lambda \rangle$.
% We use the operator $\odot$ to denote a string $e \in \Sigma^*$ plugged into a context: $e \odot \langle l, r \rangle = ler$.

\subsection{Meaning}

We assume the existence of a \emph{denotational semantics} over every substring of $L$, which we now elaborate on.
Let $Y$ be a countable set of referents.
First, we will say that some $e \in \Sigma^*$ is a valid \emph{expression} within the context $\kappa = \langle l, r \rangle$ if there exists some contextual denotation $\den{e \mid \kappa} \in Y$. Intuitively, this represents the value of $e$ when it occurs in the larger context $ler \in L$. We will also use the notation $\den{e \mid l, r}$ where convenient.
% We assume the existence of a grammar function $G(e \mid \kappa)$ that tells us whether $e$ is an expression in $\kappa$.
We will reserve $\emptyset \in Y$ as a special null symbol. Iff $e$ is not a valid expression in the context $\kappa$, we define $\den{e \mid \kappa} = \emptyset$.\footnote{\upd{Note that the simple model of denotations we use here does not reflect the range of semantic theories that have been proposed for natural language. In particular, our denotations $\den{e \mid \kappa}$ depend only on the linguistic context $\kappa$ rather than any external world state. This differs substantially from how truth conditions are traditionally conceptualized in formal semantics \citep{Heim1998-HEISIG}. For example, in our framework, the referent of English $\den{\textit{the dog} \mid \kappa}$ could not depend on any world state to determine which dog is contextually salient. \autoref{sec:towards-nl} further discusses the differences between our setup and the richer semantics of natural language.}}

Let $E(L)$ denote the set of all expressions that can appear in at least one valid context within the language $L$.
Each string $e \in \Sigma^*$ also has a \emph{support}, or a set of contexts where it is a valid expression:
\begin{equation}
    \supp_L(e) = \{ \kappa \in (\Sigma^*)^2 \mid \den{e \mid \kappa} \neq \emptyset \} .
\end{equation}
\noindent We will refer to a set of contexts $S \subseteq (\Sigma^*)^2$ as a \emph{syntactic role}. Each syntactic role has a set of expressions $E(S)$ whose support is that role:
\begin{equation}
    E(S) = \{ e \in E(L) \mid \supp_L(e) = S \} .
\end{equation}

% Further, for every $e \in \Sigma^*$, \footnote{$\den{e}$ is defined for any $e \in \Sigma^*$ but reduces to $\{ \langle \kappa, \emptyset \rangle \mid \kappa \in (\Sigma^*)^2 \}$ unless $e$ is a valid expression in some $\kappa$.}
Further, for every $e \in E(L)$, we define the (uncontextualized) \textit{denotation} of $e$ as
\begin{equation} \label{eq:gen-meaning}
    \den{e} = \{ \langle \kappa, \den{e \mid \kappa} \rangle \mid \kappa \in (\Sigma^*)^2 \} .
\end{equation}
% \noindent For a support $D \subseteq (\Sigma^*)^2$, we write $\den{e}_D$ to denote the meaning of $e$ within the contexts of $D$:
% \begin{equation}
%     \den{e}_D = \{ \langle a, z, m \rangle \in \den{e} \mid \langle a, z \rangle \in D \} .
% \end{equation}

% \roy{Shouldn't it be $\kappa \in \supp_L(e)$? I see that later in the example you say that it does include contexts that are not well-formed, but maybe it's best to mention it here}
\noindent
Recall that $\den{e \mid \kappa} = \emptyset$ for ill-formed contexts $\kappa$, which is why \eqref{eq:gen-meaning} is defined for all $\kappa \in (\Sigma^*)^2$.
Whereas $\den{\cdot \mid \kappa}$ represents the contextualized meaning representation for an expression, $\den{\cdot}$ represents its \textit{general meaning}.

\paragraph{Example} We introduce a concrete example of this formal model.
Let $L$ be a language of integers and along with the \pythoninline{+} operator, e.g., \pythoninline{2 + 2}. We take $\den{e \mid \kappa}$ to map $e$ to its standard arithmetic interpretation, i.e., $\den{\pythoninline{2 + 6} \mid \lambda, \pythoninline{+ 4}} = 8$.
We take expressions that are not conventionally well-formed to be invalid: e.g., $\den{\pythoninline{+} \mid \lambda, \pythoninline{+}} = \emptyset$.
Then $\supp_L(\pythoninline{2})$ is the set of all contexts where a $\pythoninline{2}$ can occur as a valid expression, which includes $\langle \lambda, \pythoninline{+ 4} \rangle$.
Since the value of \pythoninline{2 + 6} does not change depending on context, $\den{\pythoninline{2 + 6}}$ is the set of tuples of the form $\langle \kappa, 8 \rangle$ if $\kappa$ is a syntactically well-formed context, and $\langle \kappa, \emptyset \rangle$ otherwise.
% \begin{equation}
%     \begin{cases}
%     \langle \kappa, 8 \rangle & \textrm{if} \; aez \in L \\
%     \langle a, z, \emptyset \rangle & \textrm{otherwise.}
%     \end{cases}
% \end{equation}
$Y$ is simply the integers.

\subsection{Comparing Meanings}

Let $\rel$ be a semantic relation defined over elements of the set $Y$.
We will extend $\rel$ from $\den{e \mid \kappa} \in Y$ to general meaning $\den{e}$ in the natural way.
For two expressions that occur in the same contexts, we will enforce that $\rel$ holds in every context:

\begin{definition}[Semantic comparison] \label{def:equal-hat}
Consider $e, e' \in E(L)$ and a relation $\rel : Y^2$. We say that $\den{e} \rel \den{e'}$ iff, for all $\kappa \in (\Sigma^*)^2$,
\begin{align*}
    \den{e \mid \kappa} &= \den{e' \mid \kappa} = \emptyset \\
    \vee \quad \den{e \mid \kappa} &\rel \den{e' \mid \kappa} .
\end{align*}
% Consider $e, e' \in E(L)$, and let $S = \supp_L(e) \cap \supp_L(e')$.
% We compare two general meanings using the relation $\equalhat$, which is defined according to
% \begin{align*}
%     \den{e} \equalhat \den{e'} \iff S \neq \emptyset \; \wedge \\
%     \forall \kappa \in S, \; \den{e \mid \kappa} = \den{e' \mid \kappa} .
% \end{align*}
\end{definition}

\noindent Informally, this says that $\rel$ must hold in every shared context, and that there cannot be any unshared contexts. In particular, we will focus on the case where $\rel$ is the semantic equivalence relation $=$. \upd{In this case, \autoref{def:equal-hat} is equivalent to the conventional meaning of $=$ over sets, i.e., that each set contains the same elements. Extending our running example of an algebraic language over integers, we would have that $\den{\pythoninline{4 + 4}} = \den{\pythoninline{8}}$.}
% If we let $\rel$ be the $<$ relation, it would also be the case that $\den{\pythoninline{7}} < \den{\pythoninline{8}}$.

\subsection{Referential Transparency}

As defined above, we make very few assumptions about denotations.
They are not necessarily compositional, and meaning may be influenced by ``side effects'' of the context.
However, we saw in the example language of integer expressions that the meanings of expressions did not depend on the context at all.
We now define a property of $\den{\cdot}$ that formalizes this idea.

% https://stackoverflow.com/questions/4865616/purity-vs-referential-transparency

% TODO: Can just define null outside support of L.

\begin{definition}[Referential transparency] \label{def:ref-trans}
An expression $e \in E(L)$ is \emph{referentially transparent} iff, for all $\kappa \in (\Sigma^*)^2$, either $\den{e \mid \kappa} = \den{e \mid \lambda^2 } \neq \emptyset$, or $\den{e \mid \kappa} = \emptyset$.
\end{definition}

\noindent Informally, this says that $e$ has a well-defined denotation that exists independent of context, and that this simple denotation can be ``plugged into'' any context.
% \footnote{\autoref{def:ref-trans} is slightly stronger than other definitions of referential transparency, which say that every occurrence of $e$ within a specific \emph{syntactic role} must have a well-defined denotation. We choose this version because the distinction is irrelevant to our arguments, and we wish to remain theory-neutral with respect to syntactic formalisms.}
% \autoref{def:ref-trans} immediately implies that $\den{\cdot \mid a,z} \cong_= \den{\cdot}$.
Our previous example expression $\pythoninline{2 + 6}$ is fully referentially transparent because it can be said to have a well-defined value $8$ independent of its context. We could break referential transparency by adding bound variables to the language, e.g. \pythoninline{x = 2; x + 6} in Python. In this case, $\den{\pythoninline{x} \mid \kappa}$ \upd{non-vacuously} depends on $\kappa$.

\subsection{Assertion Queries}

% We formalize the type of knowledge a system 
We now define an oracle function providing assertion information about expressions in $L$, resembling \pythoninline{assert e1 == e2} for two Python expressions \pythoninline{e1}, \pythoninline{e2}. A system is granted access to this function, and it can make \textit{assertion queries} to it in order to learn about the semantics of $L$.\footnote{This resembles the role of queries in classical grammar induction works \citep[e.g.,][]{angluin1987queries}.}
An assertion query tells us whether two expressions $e, e'$ are equivalent within the context $\kappa$.

% We allow this oracle to take arbitrary strings, not just expressions.
\begin{definition}[Assertion oracle]
For $e, e', \in \Sigma^*$ and $\kappa \in (\Sigma^*)^2$, define the \emph{assertion oracle}
\begin{equation*}
    \assert_=(e, e' \mid \kappa) =
    \begin{cases}
        % \emptyset & \textrm{if} \; aez \notin L \; \textrm{or} \; ae'z \notin L \\
        1 & \textrm{if} \; \den{e \mid \kappa} = \den{e' \mid \kappa} \\
        0 & \textrm{otherwise} .
        % 1 & \textrm{if} \; \mu^w(e)(a, z) = \mu^w(e')(a, z) \\
        % \emptyset & \textrm{otherwise} .
    \end{cases}
\end{equation*}
\end{definition}

% We use the empty set $\emptyset$ as an ``undefined'' symbol for queries that fall outside the domain of $L$.
Recall that we defined $\den{e \mid \kappa} = \emptyset$ if $e$ is not valid in the context $\kappa$. 
In our example language of integer expressions, for all $\kappa$,  $\assert_=(\pythoninline{4}, \pythoninline{2 + 2} \mid \kappa) = 1$, since $4 = 2 + 2$. The computational power of this oracle depends on the complexity of the underlying semantics: for arbitrary complex semantics, it can become uncomputable.

The $\assert_=$ oracle is motivated by assertion operators in programming languages, which occur naturally in environments like unit tests.
The distribution of strings in a corpus of code should capture some notion of this oracle,
since a programmer is more likely to assert two expressions are equal if they are expected to have the same value.
% since expressions are more likely to be asserted equal if they
% \nascomment{modified here, might clarify Roy's misunderstanding, please check} are expected by the programmer to have the same value.\roy{I am not sure I understand this statement. they are surely asserted equal if they have the same value, aren't they? and how does this relate to the distribution of strings? I was expecting some sort of argument that relates to the distributional semantics hypothesis (e.g., they are likely to be asserted true if they appear in similar contexts}
Our goal is to study the limits of understanding achievable from raw text, so we consider an ``upper bound'' setup by assuming a system has full access to $\assert_=$.
% To explore an ``upper bound'' on the understanding achievable by a language model, we imagine that it has full access to $\assert_=$.
Even with access to this powerful oracle, is it possible for the system to emulate the underlying semantics in a way that preserves semantic relations?

\subsection{Emulation}

Finally, several concepts are necessary for our definition of semantic emulation, coming in \autoref{sec:question}.
We formalize semantic emulation in terms of \emph{isomorphism} between functions over strings with respect to semantic relations.

\begin{definition}[Isomorphism] \label{def:isomorphism}
Let $E \subseteq \Sigma^*$ be a generic set of strings.
Let $F, G$ be two sets, each equipped with a binary relation $\rel$.
Consider $f : E \rightarrow F$ and $g : E \rightarrow G$.
We say that $f,g$ are \emph{\isomorphic} w.r.t. $\rel$ over $E$ iff, for all $e, e' \in E$,
% Can define this equivalence "over L"
\begin{equation*}
    f(e) \rel f(e') \iff g(e) \rel g(e') .
\end{equation*}
\noindent We write $f \cong_\rel g$ iff $f, g$ are \isomorphic w.r.t. $\rel$.
\end{definition}

This is the definition of isomorphism over relational structures in algebra, where the sets in question are $F,G$: the images of $E$ under $f,g$.
As with \autoref{def:equal-hat}, we will focus on the case where $\rel$ is $=$. However, we can also let it refer to other relations like as ``entailment'', which we explore in \autoref{sec:other-relations}.
Note that, for any $\rel$, $\cong_\rel$ always satisfies the conditions for an equivalence relation. This means any function $f$ will always belong to a well-defined equivalence class under $\cong_\rel$.

Computing an isomorphism of $\den{\cdot}$ under the semantic relation $\rel$ can be thought of as emulating meaning representations that preserve $\rel$.
For example, recall our example language of integer expressions.
If a function $\mu \cong_= \den{\cdot}$, then $\mu$ will consider two expressions to be equivalent exactly when they evaluate to the same integer.

Another important component of our conditions for emulation is computational realizability.
We will use Turing machines \citep{turing1936computable} as a model of universal computation.
We say that a relation $\rel : M^2$ is \textit{decidable} over $M$ if there exists a Turing machine $T$ such that, for every $m, m' \in M$, $T$ halts and computes the boolean value of $m \rel m'$ on input $\langle m, m' \rangle$. Similarly, for $E \subseteq \Sigma^*$, we say that $f : E \to M$ is \emph{computable} over $E$ if there exists a Turing machine $T$ that outputs $f(e)$ on input $e \in E$. We will also define an oracle Turing machine $T$ as a standard machine that can compute a blackbox ``oracle'' function $f$ as a subroutine. We imagine $T$ has a special \emph{query} instruction and tape. After writing $x$ to the query tape and executing the query instruction, the query tape will contain $f(x)$.
Whereas, in computability theory, oracle Turing machines are generally leveraged to make reductions from uncomputable problems, here we will use them to formalize the ability of an emulator to make assertion queries about $L$. This oracle provides additional power because these queries provide additional information beyond that encoded in the input expression.

% In \autoref{sec:explain-iso}, we explain how this notion of isomorphism constitutes an isomorphism in the standard algebraic sense.

==> v1/question.tex <==
\section{Research Question: Do Assertions Enable Understanding?} \label{sec:question}

There is a long history in AI of trying to define and measure understanding. \citet{turing1950computing} constitutes an early \upd{behaviorist} perspective; more recent approaches tend to emphasize not just an external view of a system's behavior, but also ``how it is achieved'' \citep{levesque2014}. 
Understanding can be behaviorally diagnosed in neural models by evaluating them on benchmarks \citep{wang-etal-2018-glue}.
An alternate approach is probing \citep{adi2017fine, conneau-etal-2018-cram, ijcai2018-796, hewitt-liang-2019-designing, belinkov2019analysis}, which investigates \textit{how directly} a model's representations encode semantic relations by measuring if they can be easily decoded from them.
Similarly, 
we take the position that systems are capable of understanding if they \emph{emulate} representations that are isomorphic to underlying meaning under important semantic relations like equivalence. We will formalize this in \autoref{qu:computing-meaning}, which asks whether such emulation is possible using assertions.


First, we justify that an assertion oracle uniquely determines the equivalence class of meaning representations that are isomorphic to $\den{\cdot}$ within each syntactic role $S$. It follows from \autoref{def:equal-hat} that,
for all $e, e' \in E(L)$,
\begin{align} \label{eq:well-defined}
    &\forall \kappa \in (\Sigma^*)^2, \; \assert_=(e, e' \mid \kappa) \\
    &\iff \den{e} = \den{e'}.
\end{align}
\noindent Thus, the equivalence class of $\den{\cdot}$ under $\cong_{=}$ (the goal of our emulation) is uniquely defined by $\assert_=$.
However, the quantification over contexts in \eqref{eq:well-defined} is potentially infinite.
A question remains about whether it is possible to \emph{compute} (in finite time) some representative $\mu$ from this equivalence class.
To address this question, we now formally define what we mean by ``emulation'':

\begin{definition}[Emulation] \label{def:emulation}
A meaning representation $\mu : E(L) \rightarrow M$ emulates $\den{\cdot}$ w.r.t. $=$ iff:
\begin{compactenum}
    \item $\mu \cong_{=} \den{\cdot}$ over $E(S)$ for each $S \subseteq (\Sigma^*)^2$ \label{cond:isomorphic}
    \item $=$ is decidable over $M$ \label{cond:decidable}
    \item $\mu$ is computable over $E(L)$ by a Turing machine with oracle access to $\assert_=$. \label{cond:computable}
\end{compactenum}
\end{definition}

Emulation extends isomorphism, enforcing the constraint that the representation $\mu$ is computationally realizable with access to assertion queries. Also note that it enforces isomorphism only between expressions of a particular syntactic role, which are directly comparable, rather than generally. We are ready to formally state the research question about a formal language $L$ with denotational semantics $\den{\cdot}$:

\begin{question} \label{qu:computing-meaning}
Does there exist $\mu : E(L) \rightarrow M$ such that $\mu$ emulates $\den{\cdot}$ w.r.t. $=$?
\end{question}

% Note that we are applying the notion of isomorphism from \autoref{def:isomorphism} to meaning functions.
% As meaning is not directly observed in our setup, $\cong_=$ can be viewed as a form of \emph{observational equivalence}, i.e., a relation under which two meaning representations are identical if it is impossible to distinguish them through observations in the form of queries to $\assert_=$.\roy{I think this definition of meaning should not be hidden in this paragraph, but made more explicit. it seems key to the arguments}

How does \autoref{qu:computing-meaning} relate to understanding in large language models? We imagine that, with sufficiently large amounts of data, the frequencies of strings in $L$ carry enough signal such that a language model viewing enough strings can
% directly compute $\member$ and can
simulate $\assert_=$.
% \roy{it feels like we should be citing (Harris, 1955) somewhere here}
In other words, assume that the distributional properties \citep{harris1954distributional} of $L$, which capture contexts like unit tests, us whether two expressions \upd{denote the same referent} in a specific context. The question we are asking, then, is whether this would allow a language model to emulate accurate semantic representations for all expressions, i.e., compute some isomorphism to $\den{\cdot}$. Using isomorphism abstracts away from the lack of direct grounding, allowing us to ask questions about whether an ungrounded system can \textit{emulate} representations that preserve underlying semantic relations.

Stepping back, \autoref{qu:computing-meaning} bears on the role of assertions raised by \citet{bk-2020}. Does observing assertions allow a Turing-complete system to emulate a compiler? \upd{In more general terms, are assertions powerful enough implicit grounding to achieve representations that encode the denotational semantics of a language?}

==> v1/side_effects.tex <==
\section{Side Effects} \label{sec:side-effects}

Removing the condition of referential transparency,
spans in the text can have \emph{side effects}, changing the meaning of other spans of text. This allows operations like assigning variables in Python, or binding pronouns in natural language. We show that these side effects can make emulating meaning uncomputable. \upd{In particular, we show an example of a Python fragment $L_P$ over which no emulator $\mu$ is Turing-computable.}

\begin{definition}[$L_P$ syntax and semantics] \label{def:template}
We define the language $L_P$ as the set of strings specified in \autoref{fig:template}, where $n,m$ are metavariables ranging over all natural numbers serialized as decimal strings.
% \roy{to make sure I understand, the template strings are the actual python strings? it is quite confusing to look at these lines of code and consider them as templates}
For $ler \in L$, we define $\den{e \mid l, r}$ as the value of $e$ evaluated within the larger program $ler$ according to standard Python 3.8 semantics. If the substring $e$ is not a valid Python expression in the context $\langle l, r \rangle$, then $\den{e \mid l, r} = \emptyset$.

Assume a function \pythoninline{tm\_step(config: int) -> int} has been defined in the global namespace, taking a natural number representing a configuration (tape contents and finite state) for a universal Turing machine, and returns the configuration that results from running one step of computation. The \pythoninline{config} value $0$ is reserved as a special symbol representing a halted machine.
\end{definition}
% \yg{From my experience with PL people, they are always very worried about proving things about a ``real'' programming language like python. They alwasy uses purer, and much simpler, languages. There is probably a reason for that, they've been burnt by this before. But, even if your proof is fully correct, I fear that once a PL person sees this they will become immediately super skeptical about it. Can you use a simple language to make your point?} 

% \nascomment{maybe give some intuition about what's in ``$w$''?}

The idea behind $L_P$ is to construct a language where the oracles are computable, but $=$ cannot be decided over $Y$. Thus, there is no way to compute an isomorphic representation $\mu : E(L) \rightarrow M$ such that $=$ can be decided over $M$ without making $\mu$ uncomputable. We now formalize this.

\begin{figure*}

\begin{minipage}{.5\textwidth}
\centering
\begin{python}
def tm_run(config: int) -> int:
    for _ in range($\color{red} n$):
        config = tm_step(config)
    return config

print(tm_run($\color{red} m$) == 0)
\end{python}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\centering
\begin{python}
def tm_run(config: int) -> int:
    for _ in range($\color{red} n$):
        config = tm_step(config)
    return config

print(False)
\end{python}
\end{minipage}

\caption{Templates for strings in $L_P$, with metalinguistic elements in red. $L_P$ contains all strings matching either template, with metavariables $n,m$ range over all natural numbers, serialized as decimal strings. Let \pythoninline{tm\_step} be a function that runs one step of Turing machine computation, returning the new config.}
    \label{fig:template}
\end{figure*}

\begin{theorem}[Non-transparency] \label{thm:side-effects}
Consider the syntax and semantics of $L_P$ from \autoref{def:template}.
% Let $S = \supp_L(\pythoninline{False})$.
Then, there exists no $\mu : E(L) \rightarrow M$ such that $\mu$ emulates $\den{\cdot}$ w.r.t. $=$.
% For all $\mu : E(L) \rightarrow M$ such that
% $\mu$ emulates $\den{\cdot}$ w.r.t. $=$ over $\suppset{D}_L$,
% there exists no Turing machine with oracle access to $\assert_=$
% such that, for $e \in E(L)$, $T$ computes $\mu(e)$ on input $e$.
\end{theorem}

\begin{proof}
We present a template for strings in $L_P$ in \autoref{fig:template}.\footnote{$L_P$ can be viewed as a concrete formal model of Python.}
Crucially, $\den{e \mid l, r}$ can be computed on any $ler \in L_P$ because $n$ is finite. Thus, $\assert_=(e, e' \mid l, r)$ can be computed for any setting of its arguments.
% $x \in L_P$ can also be easily checked for any $x$. Thus, $\member$ is also computable.

We want to compute some $\mu$ such that all the emulation conditions hold. First, it must be the case that $\mu \cong_{=} \den{\cdot}$ (\autoref{cond:isomorphic}).
Since we have established the oracles are computable, the Turing machine computing $\mu$ (\autoref{cond:computable}) is no more powerful than a general Turing machine. By \autoref{cond:decidable}, it must also be the case that $\mu(e) \stackrel{?}{=} \mu(e')$ is decidable for all $e, e' \in E(L)$. Combining these conditions, it needs to be decidable by a general Turing machine whether, for every $m$,
\footnote{We use red italics for metavariables in Python code.}
\begin{equation} \label{eq:iso-question}
    \den{\pythoninline{tm\_run($\color{red} m$) == 0}} \stackrel{?}{=} \den{\pythoninline{False}} .
\end{equation}

For every $n,m \in \mathbb{N}$, let $\kappa_{n,m} \in (\Sigma^*)^2$ denote the context shared by the two templates in \autoref{fig:template}, excluding the differing expressions (\pythoninline{tm\_run($\color{red} m$) == 0} versus \pythoninline{False}).
We let $S$ be the set of all these contexts.
\eqref{eq:iso-question} is equivalent to deciding whether, for all $n,m$,
\begin{align} \label{eq:den-question}
    \den{\pythoninline{tm\_run($\color{red} m$) == 0} \mid \kappa_{n,m}} \\
    \stackrel{?}{=} \den{\pythoninline{False} \mid \kappa_{n,m}}
    = \pythoninline{False} .
\end{align}
% \noindent For all $n,m$, $\den{\pythoninline{False} \mid a_{n,m}, z_{n,m}} = \pythoninline{False}$. Thus, \eqref{eq:den-question} reduces to
% \begin{equation}
%     \den{\pythoninline{tm\_run($\color{red} m$) == 0} \mid a_{n,m}, z_{n,m}} \stackrel{?}{=} \pythoninline{False} .
% \end{equation}

\noindent This entails deciding whether, for all $m$, the universal Turing machine with initial state $m$ ever halts, i.e., the ``halting problem''. This problem cannot be decided by a Turing machine for all inputs \citep{turing1936computable}.

In summary, we have shown that $\assert_=$ is computable, giving the emulator $\mu$ no more power than a standard Turing machine. Thus, computing $\mu$ cannot be reduced to making assertion queries. Either $\mu$ becomes uncomputable, or the relation $=$ is undecidable over $E(S)$.
% Note: can get rid of dependence on $w$ by putting config value in a metavariable $m$, rather than doing djanky standard input thing.
\end{proof}

\subsection{Discussion}

We provide a brief summary of this result in less formal terms.
Every program in $L_P$ halts---we are not constructing programs that do not halt. With knowledge of the Python interpreter, any agent could execute all of these programs. Rather, what we have shown is that, with finite time, it is impossible for an ungrounded agent to simulate the Python interpreter \textit{using assertion queries}. In other words, without prior knowledge of the interpreter or some kind of grounding, no algorithm can use queries to disambiguate which notion of $=$ Python uses from the infinite other possibilities.

\autoref{thm:side-effects} should not be mistaken for a family of arguments about the difficulty of language modeling that reduces uncomputable or intractable problems to language modeling. For example, one could input a prompt \emph{There is a universal Turing machine with initial configuration $\color{red} m$. Does the machine halt? The answer is..}. 
In that case, predicting the next token requires solving the halting problem, suggesting that arbitrary language modeling is uncomputable. That is \emph{not} the argument we are making. In our case, each program in $L_P$ \emph{can} be evaluated with access to an interpreter. Rather, we show that it is impossible for an ungrounded Turing-complete system to figure out how to interpret them. Crucially, we do not rest on the assumption that language models should be able to make inferences requiring arbitrary computational power.\footnote{\autoref{thm:side-effects} says that it is impossible to understand each expression \pythoninline{tm\_run($\color{red} m$) == 0} for \emph{all} $m$. However, it is possible to emulate understanding for \emph{most} of them, in a particular formal sense. This is because the halting problem is almost surely decidable as the number of states of a Turing machine goes to infinity \citep{hamkins2006}. However, this is not a desirable way to measure probability over Turing machines, as, under the same view, Turing machines almost surely recognize only a finite language. Infinite formal languages, the main object of study in formal language theory, would only appear with probability $0$.}$^{,}$\footnote{Another view is not just whether it is possible to emulate $\den{e}$, but what the computational complexity of this emulation is. Fixing integers $n, m$, an algorithm like \autoref{fig:countable} can be used to emulate understanding on expressions with length $< n$ within contexts of lengths $< m$ for any language. Doing this requires at worst $\mathcal O(\abs{\Sigma}^{nm})$ assertion queries. See \citet{pratt-hartmann2006} and other works in semantic complexity for different yet relevant results about the computational complexity of understanding fragments of natural language.}

While it is more precise to state \autoref{thm:side-effects} in a formal language resembling Python, an argument similar to \autoref{thm:side-effects} can be adapted to a natural language like English. An example is shown in \autoref{fig:english-template}, where we define the meaning of a sentence as its truth conditions.
% The truth conditions of the third sentence are analogous to the return value in \autoref{fig:template}.
Deciding if \emph{$\color{red} m$ halted} has the same truth conditions as \emph{Zero equals one} for all $m$ requires solving the halting problem. A system must necessarily fail to emulate the semantics of these expressions.
The rest of the paper \upd{further explores} the implications and limitations of applying our formal model to natural language.

\begin{figure*}

\begin{minipage}{.5\textwidth}
\centering
\begin{lstlisting}[mathescape=true,frame=tb,basicstyle=\small]
There is a Turing machine $\color{red} m$.
It ran for $\color{red} n$ steps.
$\color{red} m$ halted.
\end{lstlisting}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\centering
\begin{lstlisting}[mathescape=true,frame=tb,basicstyle=\small]
There is a Turing machine $\color{red} m$.
It ran for $\color{red} n$ steps.
Zero equals one.
\end{lstlisting}
\end{minipage}

% \begin{lstlisting}[mathescape=true,frame=tb]
% There is a Turing machine $\color{red} m$.
% The machine ran for $\color{red} n$ steps.
% $\color{red} \{m$ halted.$\color{red} ,$Zero equals one.$\color{red} \}$.
% \end{lstlisting}
    \caption{An informal construction adapting the program templates in \autoref{fig:template} to English. \upd{Under our framework, two sentences are considered equivalent if they are true in exactly the same set of contexts. Deciding whether the final lines of the two templates are equivalent for all $m$ entails solving the halting problem.}}
    \label{fig:english-template}
\end{figure*}

% \nascomment{the English version is great!}

==> v1/subroutines.tex <==
\begin{figure*}
    \centering
    \begin{python}
from itertools import count, product
from typing import Iterable

def all_strings() -> Iterable[str]:
    for length in count():
        iterable = product(*[SIGMA for _ in range(length)])
        yield from ("".join(x) for x in iterable)
    \end{python}
    \caption{An concrete implementation of \pythoninline{all\_strings}, which is referenced in \autoref{fig:countable} and \autoref{fig:extended-countable}.}
    \label{fig:subroutines}
\end{figure*}

% \section{Enumeration Subroutine} \label{sec:subroutines}

% In \autoref{fig:countable}, we define a subroutine for iterating over strings that was referenced in the main body.

% def all_triples() -> Iterable[Tuple[str, str, str]]:
%     covered = set()
%     string_iter = all_strings()
%     strings = []
%     for idx in count():
%         strings.append(next(string_iter))
%         for i, j, k in product(range(idx + 1), range(idx + 1), range(idx + 1)):
%             if (i, j, k) in covered:
%                 continue
%             yield strings[i], strings[j], strings[k]
%             covered.add((i, j, k))

==> v1/towards_nl.tex <==
\section{Towards Natural Language} \label{sec:towards-nl}

As discussed in \autoref{sec:intro}, our results are inspired by the thought experiment of whether a language model can use raw code to learn a compiler. A goal of this, of course, is to examine whether understanding can be acquired from natural language text in a simplified setting. In principle, our formal results can bear on this broader question about natural language, although some differences emerge when extending the results to a less well-defined setting. \upd{In many cases, these differences appear to make the task of learning meaning harder, suggesting that our negative claim in a simpler setting (\autoref{thm:side-effects}) may still hold as an impossibility result.} We now discuss some points of difference between our formal model and natural language.

% https://plato.stanford.edu/entries/truth/

\paragraph{Truth Conditions} For a boolean-valued expression $e$, our notions $\den{e \mid \kappa}$ and $\den{e}$ resemble the distinction drawn between truth values and truth conditions in linguistic semantics.
% \citep{frege1948sense}.
\upd{Whereas $\den{e \mid \kappa}$ represents the value of $e$ in a fixed context, $\den{e}$ can be interpreted as a function associating linguistic contexts with values of $e$. A crucial difference is that these conditions are not \emph{intensions} \citep{Fintel_intensionalsemantics}, i.e., they are not functions of the world state, but rather of the linguistic context only.} Thus, one way to rephrase \autoref{qu:computing-meaning} is whether non-intensional truth conditions can be emulated from assertion queries alone.
% \paragraph{Intensionality} Our formal model assumes that the meaning of an expression $\den{e \mid \kappa}$ can only depend on its linguistic context $\kappa$: not any state of the external world.
% % (which we might represent as $w$).
This model is natural for formalizing a closed programming language environment, e.g., with no environment variables or user input, \upd{since in this case the program state is specified completely by the linguistic context.} On the other hand, English has common elements like \textit{that} whose meaning is directly conditioned by \upd{world state external to language.} \upd{Perhaps allowing such elements would only make understanding more difficult; or, arguably, generally impossible, since there is no way for the model to observe the grounding world state using only an assertion oracle. We are inclined to believe that, since such changes would make understanding more difficult, \autoref{thm:side-effects} would still hold as an impossibility result. However, future work would be needed to make this idea precise.}

\paragraph{Possible Worlds} Programs execute in well-defined environments with a clear state. It is natural to talk about the value that is the referent of an expression. Speakers of natural language, on the other hand, have imperfect information and beliefs about the world around them. Thus, it can be more natural to model the referent of a sentence over a set of \emph{possible worlds}, rather than within a specific evaluation context. In \autoref{sec:modal}, we explore to what degree this setting makes the task of learning to understand more difficult. In adapting our model to this context, the assertion oracle must become ``modal'' in the sense that it quantifies over sets of worlds. We explore two different models of modality for the oracle, corresponding to different physical interpretations. In one case, \autoref{thm:transparency} and \autoref{thm:side-effects} apply analogously, while, in the other, emulation becomes an ill-defined problem.

% \paragraph{Pragmatics}
\paragraph{Denotation vs.~Intent} \citet{bk-2020} distinguish between \emph{standing meaning} and \emph{communicative intent}, reflecting a distinction between denotational semantics and other pragmatic intentions that a speaker has in producing an utterance. In this paper, it is most straightforward to imagine $\den{e}$ reflecting standing meaning. In principle, we could imagine that it represents the speaker's communicative intent, and that an omniscient oracle $\assert_=$ can reveal information about the speaker's intents to the system. Even with this unrealistically powerful oracle, \autoref{thm:side-effects} says that learning to emulate the speaker's intents is impossible for a Turing-complete system.

\paragraph{Other Relations} \autoref{thm:transparency} and \autoref{thm:side-effects} investigate whether $\assert_=$ can be used to emulate meaning representations that preserve an equivalence relation. While equivalence is an important part of semantics, other semantic relations like entailment are also necessary for language understanding. In \autoref{sec:other-relations}, we show a generalization of \autoref{thm:all-rel} extends to \emph{any} semantic relation. In other words, referential transparency also enables emulation of relations besides $=$.

\paragraph{Competence vs.~Performance} \citet{chomsky2014aspects} differentiates competence and performance in linguistic theory, where competence corresponds roughly to the correct algorithmic modeling of a linguistic process, and performance describes its implementation subject to resource constraints like memory. Arguably, agents might be said to understand language if they are competent in this sense, even if they sometimes make performance errors. In contrast, our definition of emulation (\autoref{def:emulation}) permits no performance errors. In future work, it would be interesting to adapt an approximate notion of emulation that tolerates performance errors in order to more closely target understanding in a sense reflecting competence.

==> v1/transparent.tex <==
\section{No Side Effects} \label{sec:no-side-effects}
We first consider the case where all expressions are referentially transparent, which is equivalent to saying that there can be no side effects. In this case, \autoref{thm:transparency} will show that it is always possible to use assertion queries to emulate $\den{\cdot}$. \upd{The core idea of the proof is to construct a canonical form for each expression. The canonical form is the first expression in a lexicographic ordering that the assertion oracle deems equivalent to the target expression. For technical reasons, the emulator returns the index of this string under the lexicographic order.}

% For notational convenience, we will omit the $a, z$ arguments of $\assert_=$, which are vacuous by referential transparency. In other words, we will write $\assert_=(e, e')$ instead of $\assert_=(e, e' \mid a, z)$.
% \autoref{qu:ref-trans} is answered by the following result:

% SyntaxType = Callable[[str, str, str], bool]


\begin{figure*}
    \centering
    \begin{python}
from typing import Callable

AssertType = Callable[[str, str, str, str], bool]

def emulate(expr: str, ass_equals: AssertType) -> int:
    for idx, cand in enumerate(all_strings()):
            if ass_equals(expr, cand, "", ""):
                return idx
    \end{python}
    \caption{Given $e \in E(L)$, \pythoninline{emulate} computes $\mu$ such that $\mu$ emulates $\den{\cdot}$ w.r.t. $=$. Let \pythoninline{all\_strings} be an iterable enumerating all strings in $\Sigma^*$. We provide a concrete implementation of \pythoninline{all\_strings} in \autoref{fig:subroutines}.}
    \label{fig:countable}
\end{figure*}
% # Assume all_strings is an iterable over $\Sigma^*$.

\begin{theorem}[Transparency] \label{thm:transparency}
Consider $L$ such that each $e \in E(L)$ is referentially transparent. Then, there
exists $\mu : E(L) \rightarrow \mathbb{N}$
such that $\mu$ emulates $\den{\cdot}$ w.r.t. $=$.
% exists $\mu \cong_= \den{\cdot}$
% and some Turing machine $T$ with oracle access to $\assert_=$
% % and $\member$
% such that:
% % for each support $D \subseteq (\Sigma^*)^2$,
% % $\mu$ emulates $\den{\cdot}$ w.r.t. $=$ over $\suppset{D}_L$,
% % % $\mu \cong_= \den{\cdot}$,
% % % $=$ is decidable over $M$,
% % and, for all $e \in E(L)$, $T$ computes $\mu(e)$ on input $e$.
% \begin{compactenum}
%     \item $\mu \cong_{=} \den{\cdot}$
%     \item $=$ is decidable over $M$
%     \item for all $e \in E(L)$, $T$ computes $\mu(e)$ on $e$.
% \end{compactenum}
\end{theorem}

\begin{proof}
As Python is Turing-complete, we write $\mu : E(L) \rightarrow \mathbb{N}$ as a Python function \pythoninline{emulate} in \autoref{fig:countable}. The function receives as input an expression \pythoninline{expr} and a callback function \pythoninline{ass\_equals} to an oracle computing $\assert_=$. For each $e \in E(L)$, there exists $e^* \in \Sigma^*$ such that $\assert_=(e, e^* \mid \lambda^2) = 1$. In the ``worst case'', this holds when $e^* = e$ by symmetry. By construction, \pythoninline{all\_strings} reaches all strings in finite time. Therefore, the number of loop iterations before reaching $e^*$ is finite. We can conclude that \pythoninline{emulate} halts on every $e \in E(L)$, establishing \autoref{cond:computable}.

The function \pythoninline{emulate} outputs $i \in \mathbb{N}$, the index of the first triple $e^*$ such that
\begin{align}
    % ae^*z &\in L \label{eq:part1} \\
    \den{e \mid \lambda^2 } &= \den{e^* \mid \lambda^2 } . \label{eq:part2}
\end{align}
The relation $=\ : \mathbb{N}^2$ is clearly decidable (\autoref{cond:decidable}).
So far, we have analyzed \pythoninline{emulate} applied to a single input expression $e \in E(S)$ within a syntactic role $S$.
Now, let $e, e' \in E(S)$ be two different inputs to $\mu$ within $S$.
Because the enumeration order of the \pythoninline{for} loop is fixed across computation of $\mu(e)$ and $\mu(e')$:
\begin{align}
    &\mu(e) = \mu(e') \\
    &\iff \den{e \mid \lambda^2} = \den{e^* \mid \lambda^2} \\
    &\quad \quad \wedge \den{e' \mid \lambda^2} = \den{e^* \mid \lambda^2} \label{eq:pre-equiv-rel} \\
    &\iff \den{e \mid \lambda^2} = \den{e' \mid \lambda^2} \label{eq:equiv-rel} .
\end{align}
\noindent By referential transparency, this is equivalent to saying $\den{e \mid \kappa} = \den{e' \mid \kappa}$ for any valid context $\kappa$.
We conclude $\mu \cong_{=} \den{\cdot}$ over $E(S)$ (\autoref{cond:isomorphic}).
\end{proof}

Through a simple construction,
we have shown it is possible to emulate meaning from assertion queries for languages with referentially transparent semantics. In the next section, we consider what happens without referential transparency, where context can have side effects on the meaning of an expression.
